Attributing Culture-Conditioned Generations to Pretraining Corpora

In open-ended generative tasks like narrative writing or dialogue, large language models often exhibit cultural biases, showing limited knowledge and generating templated outputs for less prevalent cultures. Recent works show that these biases may stem from uneven cultural representation in pretraining corpora. This work investigates how pretraining leads to biased culture-conditioned generations by analyzing how models associate entities with cultures based on pretraining data patterns. We propose the MEMOed framework (MEMOrization from pretraining document) to determine whether a generation for a culture arises from memorization. Using MEMOed on culture-conditioned generations about food and clothing for 110 cultures, we find that high-frequency cultures in pretraining data yield more generations with memorized symbols, while some low-frequency cultures produce none. Additionally, the model favors generating entities with extraordinarily high frequency regardless of the conditioned culture, reflecting biases toward frequent pretraining terms irrespective of relevance. We hope that the MEMOed framework and our insights will inspire more works on attributing model performance on pretraining data.

==> figures/chinese_food_heatmap.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
  \begin{center}
  \vspace{-10pt}
    \includegraphics[width=\textwidth]{images/chinese_food_heatmap_ratio.pdf}
  \end{center}
  \caption{Ratio of 25 most frequently occurring independent symbols in the pretraining corpora (y-axis) over the 25 most frequently occurring memorized symbols in the pretraining corpora (x-axis) generated by the culture ``China'' for the topic ``food''. Independent symbols appear at least as frequently and as high as 1000 times more frequently as memorized symbols.}
  \vspace{-15pt}
  \label{fig:chinese_food_heatmap}
\end{wrapfigure}

==> figures/independent_to_all.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/independent_over_all.pdf}
    \caption{Caption}
    \label{fig:independent_to_all}
\end{figure}

==> figures/independent_to_memorized.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/independent_over_memorized.pdf}
    \caption{Average ratio of counts of independent symbols over counts of memorized symbols in \dolma. The higher the ratio is, the more dominant the X-axis show 100 memorized symbols whose \huihan{change y-axis to average count of independent symbols divided by count of each memorized symbol}}
    \label{fig:independent_to_memorized}
\end{figure}

==> sections/memorization_old.tex <==
\section{Culture-centric Generations Must Contain a Health Balance of Both Memorization and Generalization}
In this section, we present a dashboard reporting statistics on the current status of culture-centric generations, and initiate a discussion on how memorization and generalization interplays with each other in the generations.

\subsection{A Dashboard}
\ti{outline:} a piechart of percentage of memorization, traceable generalization, overgeneralization, and hallucination in the generation of each country. A heatmap of percentage of memorization, traceable generalization, and how badly overgeneralization happens

\subsection{Quantifying Memorization Quality}

\paragraph{Generating Silver Ground Truth from the LLM}
We propose a methodology to generate "silver ground truth" data by leveraging the LLM, specifically using the OLMO-7B-Instruct model, to mine culturally significant symbols across various nationalities. This process begins by prompting OLMO-7B with a sequence of generation tasks designed to elicit a list of cultural symbols pertinent to specified topics and nationalities. We employ a listing-based continuation generation technique that instructs the model to enumerate items until it can no longer produce novel entries, marking the end of its output with a "DONE" token.

To enhance the relevance and uniqueness of the generated symbols and to avoid repetitive responses, we implement a constrained generation approach. This involves dynamically incorporating previously generated symbols into the model's list of "bad words" to inhibit their repetition in subsequent responses. Following the generation phase, we undertake a rigorous validation step to ground these symbols in OLMO's training documents. This grounding process serves to eliminate hallucinations and irrelevant symbols by confirming their presence and contextual relevance in the indexed data, thus establishing a robust set of "silver" ground truth data. 

\subsection{Quantifying Traceable Generalization quality}


\subsection{Quantifying Overgeneralization cultures}
